Learning Action Conditions from Instructional Manuals for Instruction Understanding

The ability to infer pre- and postconditions of an action is vital for comprehending complex instructions, and is essential for applications such as autonomous instruction-guided agents and assistive AI that supports humans to perform physical tasks. In this work, we propose a task dubbed action condition inference, and collecting a high-quality, human annotated dataset of preconditions and postconditions of actions in instructional manuals. We propose a weakly supervised approach to automatically construct large-scale training instances from online instructional manuals, and curate a densely human-annotated and validated dataset to study how well the current NLP models can infer action-condition dependencies in the instruction texts. We design two types of models differ by whether contextualized and global information is leveraged, as well as various combinations of heuristics to construct the weak supervisions. Our experimental results show a >20% F1-score improvement with considering the entire instruction contexts and a >6% F1-score benefit with the proposed heuristics.

==> figs/multi_template.tex <==
\begin{figure*}[t!]

\begin{subtable}{\textwidth}
\centering
\centering
    \includegraphics[width=.95\columnwidth]{figs/imgs/placeholder.png}
\caption{\footnotesize xxx}
\label{fig:ui_instr}
\end{subtable}

\begin{subtable}{\textwidth}
\centering
\centering
    \includegraphics[width=.95\columnwidth]{figs/imgs/placeholder.png}
\caption{\footnotesize yyy}
\label{fig:ui_ui}
\end{subtable}

\caption{ \footnotesize

}
\label{fig:ui}
\end{figure*}

==> tables/com2sense.tex <==
\begin{table*}[t!]
\centering
    \begin{tabular}{c|cccc}
    \toprule
    \textbf{Metric/Method} & \textbf{\citet{singh2021com2sense}} & \textbf{\citet{jung2022maieutic}} & \textbf{Ours New}  & \textbf{Ours New w. RP} \\
    \midrule % \\[-1.1em]
    Base Model             & UnifiedQA-3B                        & GPT-3                             & DeBERTaV3          & DeBERTaV3 \\
    \# Params              & 3B                                  & 175B                              & 304M               & 304M \\
    \midrule
    Standard (\%)          & 71.31                               & 75.00                             & \textbf{79.39}     & 82.62 \\
    Pairwise (\%)          & 51.26                               & \textbf{68.70}                    & 66.74              & 82.62 \\
    \bottomrule
    \end{tabular}
\caption{\textbf{\texttt{Com2Sense}} Performance Comparisons.
}
\label{tab:com2sense_performance}
\end{table*}

==> tables/main_results_arxiv.tex <==
\definecolor{LightCyan}{rgb}{0.88,1,1}
\newcolumntype{a}{>{\columncolor{LightCyan}}d}

\definecolor{LightGreen}{rgb}{0.9,1,0.9}
\newcolumntype{a}{>{\columncolor{LightGreen}}c}

\begin{table*}[th!]
\centering
\small
\scalebox{.93}{
    \begin{tabular}{crcc|ccc|ccc}
    \toprule
    \multicolumn{4}{c|}{\multirow{1}{*}{\textbf{\textcolor{blue}{WikiHow Annotated-Test-Set}}}} &
    \multicolumn{3}{c|}{\textbf{Precondition}} & \multicolumn{3}{c}{\textbf{Postcondition}} \\
    \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Model Type}}} & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Heuristics}}} & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Finetuned}}} & \multicolumn{1}{c|}{\multirow{1}{*}{\textbf{Self}}} & 
    Prec. & Recall & F-1 & Prec. & Recall & F-1 \\
    \midrule
    
    % Human Test Set.
    
    \multirow{2}{*}{Pairwise}
    & \multirow{1}{*}{All} & Y & N
      & 8.21 & 79.52 & 14.32 & 15.43 & 44.99 & 20.56 \\
    & \multirow{1}{*}{All} & Y & Y
      & 8.56 & \textbf{81.19} & 14.91 & 26.53 & \textbf{65.95} & 34.31 \\

    \midrule

    \multirow{8}{*}{Contextualized}
    & \multirow{1}{*}{No Heuristics} & Y & N
      & 34.01 & 58.33 & 39.27 & 34.44 & 43.15 & 36.79 \\
    & \multirow{1}{*}{No Heuristics} & Y & Y
      & 42.26 & 58.45 & 45.41 & 40.99 & 46.51 & 42.32 \\
    \cline{2-10} \\[-.8em]
    & \multirow{1}{*}{All} & N & N
      & 10.69 & 34.79 & 15.05 & 10.34 & 11.88 & 10.49 \\
    & \multirow{1}{*}{-- temporal -- coref. - keywords} & Y & N
      & 45.60 & 61.22 & 48.59 & 43.71 & 47.56 & 44.35 \\
    & \multirow{1}{*}{-- temporal -- coref.} & Y & N
      & 43.43 & 64.43 & 48.04 & 46.27 & 51.27 & 47.22 \\
    & \multirow{1}{*}{-- temporal} & Y & N
      & 45.83 & 62.48 & 49.17 & 47.72 & 52.70 & 48.81 \\
    & \multirow{1}{*}{All} & Y & N
      & 47.92 & 64.63 & 51.38 & 51.15 & 57.64 & 52.59 \\
    & \multirow{1}{*}{All} & Y & Y
      & \textbf{49.42} & 68.40 & \textbf{53.51} & \textbf{52.39} & 57.35 & \textbf{53.42} \\
    
    \midrule
    % {\color{blue}
    \multicolumn{1}{a}{\multirow{1}{*}{Human}}
    & \multicolumn{1}{a}{---} & \multicolumn{1}{a}{---} & \multicolumn{1}{a|}{---}
      & \multicolumn{1}{a}{83.91} & \multicolumn{1}{a}{83.86} & \multicolumn{1}{a|}{83.55}
      & \multicolumn{1}{a}{77.39} & \multicolumn{1}{a}{84.81} & \multicolumn{1}{a}{78.81} \\

    \bottomrule
    
    \end{tabular}
}

\centering
\small
\scalebox{.93}{
    \begin{tabular}{crcc|ccc|ccc}
    \toprule
    \multicolumn{4}{c|}{\multirow{1}{*}{\textbf{\textcolor{blue}{Instructables.com Annotated-Test-Set}}}} &
    \multicolumn{3}{c|}{\textbf{Precondition}} & \multicolumn{3}{c}{\textbf{Postcondition}} \\
    \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Model Type}}} & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Heuristics}}} & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Finetuned}}} & \multicolumn{1}{c|}{\multirow{1}{*}{\textbf{Self}}} & 
    Prec. & Recall & F-1 & Prec. & Recall & F-1 \\
    \midrule
    
    % Human Test Set.
    
    \multirow{1}{*}{Pairwise}
    & \multirow{1}{*}{All} & Y & Y
      & 6.64 & \textbf{67.13} & 11.54 & 24.53 & \textbf{61.93} & 31.78 \\
      
    \midrule

    \multirow{7}{*}{Contextualized}
    & \multirow{1}{*}{No Heuristics} & Y & N
      & 26.93 & 53.43 & 32.92 & 32.16 & 41.39 & 34.42 \\
    & \multirow{1}{*}{No Heuristics} & Y & Y
      & 38.16 & 55.77 & 42.23 & 42.57 & 48.00 & 44.07 \\
    \cline{2-10} \\[-.8em]
    & \multirow{1}{*}{-- temporal -- coref. - keywords} & Y & N
      & 39.35 & 57.03 & 43.49 & 38.45 & 42.96 & 39.39 \\
    & \multirow{1}{*}{-- temporal -- coref.} & Y & N
      & 37.06 & 59.95 & 42.56 & 38.41 & 44.54 & 39.83 \\
    & \multirow{1}{*}{-- temporal} & Y & N
      & 39.39 & 59.53 & 44.23 & 46.81 & 52.15 & 48.23 \\
    & \multirow{1}{*}{All} & Y & N
      & 40.70 & 58.97 & 45.17 & 47.92 & 56.51 & 50.06 \\
    & \multirow{1}{*}{All} & Y & Y
      & \textbf{43.81} & 62.71 & \textbf{48.34} & \textbf{53.41} & 60.51 & \textbf{55.17} \\
    
    \midrule
    % {\color{blue}
    \multicolumn{1}{a}{\multirow{1}{*}{Human}}
    & \multicolumn{1}{a}{---} & \multicolumn{1}{a}{---} & \multicolumn{1}{a|}{---}
      & \multicolumn{1}{a}{84.74} & \multicolumn{1}{a}{81.32} & \multicolumn{1}{a|}{82.78}
      & \multicolumn{1}{a}{71.90} & \multicolumn{1}{a}{82.51} & \multicolumn{1}{a}{75.53} \\

    \bottomrule
    
    \end{tabular}
}
\caption{
\footnotesize
\textbf{Annotated-test-set performance:} The best performance is achieved by applying all of the proposed \textbf{heuristics} and undergoing the two-stage training: \textbf{finetuned} on the annotated-train-set first and then perform the \textbf{self}-training. We also report ablation studies on the designed heuristics, where $^*$ -- indicates exclusion. Note that for the Instructables.com, both the \textit{Finetuned} and the \textit{Self}-training are done on the WikiHow training set and a zero-shot transfer is performed.
}
\label{tab:main_results}
\vspace{-1em}
\end{table*}

==> tables/main_results_old.tex <==
\definecolor{LightCyan}{rgb}{0.88,1,1}
\newcolumntype{a}{>{\columncolor{LightCyan}}d}

\definecolor{LightGreen}{rgb}{0.9,1,0.9}
\newcolumntype{a}{>{\columncolor{LightGreen}}c}

\begin{table*}[th!]
\centering
\small
\scalebox{.93}{
    \begin{tabular}{crcc|ccc|ccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model Type}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Heuristics}}} &
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Finetuned}}} &
    \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Self}}} 
    & \multicolumn{3}{c|}{\textbf{Precondition}} & \multicolumn{3}{c}{\textbf{Postcondition}} \\
    & & & & Prec. & Recall & F-1 & Prec. & Recall & F-1 \\
    \midrule
    
    % Human Test Set.
    
    \multirow{2}{*}{Pairwise}
    & \multirow{1}{*}{All} & Y & N
      & 8.21 & 79.52 & 14.32 & 15.43 & 44.99 & 20.56 \\
    & \multirow{1}{*}{All} & Y & Y
      & 8.56 & 81.19 & 14.91 & 26.53 & 65.95 & 34.31 \\

    \midrule

    \multirow{8}{*}{Contextualized}
    & \multirow{1}{*}{No Heuristics} & Y & N
      & 34.01 & 58.33 & 39.27 & 34.44 & 43.15 & 36.79 \\
    & \multirow{1}{*}{No Heuristics} & Y & Y
      & 42.26 & 58.45 & 45.41 & 40.99 & 46.51 & 42.32 \\
    \cline{2-10} \\[-.8em]
    & \multirow{1}{*}{All} & N & N
      & 10.69 & 34.79 & 15.05 & 10.34 & 11.88 & 10.49 \\
    & \multirow{1}{*}{-- temporal -- coref. - keywords} & Y & N
      & 45.60 & 61.22 & 48.59 & 43.71 & 47.56 & 44.35 \\
    & \multirow{1}{*}{-- temporal -- coref.} & Y & N
      & 43.43 & 64.43 & 48.04 & 46.27 & 51.27 & 47.22 \\
    & \multirow{1}{*}{-- temporal} & Y & N
      & 45.83 & 62.48 & 49.17 & 47.72 & 52.70 & 48.81 \\
    & \multirow{1}{*}{All} & Y & N
      & 47.92 & 64.63 & 51.38 & 51.15 & 57.64 & 52.59 \\
    & \multirow{1}{*}{All} & Y & Y
      & 49.42 & 68.40 & 53.51 & 52.39 & 57.35 & 53.42 \\
    
    \midrule
    % {\color{blue}
    \multicolumn{1}{a}{\multirow{1}{*}{Human}}
    & \multicolumn{1}{a}{---} & \multicolumn{1}{a}{---} & \multicolumn{1}{a|}{---}
      & \multicolumn{1}{a}{83.91} & \multicolumn{1}{a}{83.86} & \multicolumn{1}{a|}{83.55}
      & \multicolumn{1}{a}{77.39} & \multicolumn{1}{a}{84.81} & \multicolumn{1}{a}{78.81} \\

    \bottomrule
    
    \end{tabular}
}
\caption{
\footnotesize
\textbf{Annotated-test-set performance on WikiHow:} The best performance is achieved by applying all of the proposed heuristics and undergoing the second-stage self-training. We also report ablation studies on the designed heuristics, where $^*$ -- indicates exclusion.
}
\label{tab:main_results_wikihow}
\end{table*}








\definecolor{LightCyan}{rgb}{0.88,1,1}

\begin{table*}[th!]
\centering
\small
\scalebox{.93}{
    \begin{tabular}{crcc|ccc|ccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model Type}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Heuristics}}} &
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Finetuned}}} &
    \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Self}}} 
    & \multicolumn{3}{c|}{\textbf{Precondition}} & \multicolumn{3}{c}{\textbf{Postcondition}} \\
    & & & & Prec. & Recall & F-1 & Prec. & Recall & F-1 \\
    \midrule
    
    % Human Test Set.
    
    \multirow{1}{*}{Pairwise}
    & \multirow{1}{*}{All} & Y & Y
      & 6.64 & 67.13 & 11.54 & 24.53 & 61.93 & 31.78 \\
      
    \midrule

    \multirow{7}{*}{Contextualized}
    & \multirow{1}{*}{No Heuristics} & Y & N
      & 26.93 & 53.43 & 32.92 & 32.16 & 41.39 & 34.42 \\
    & \multirow{1}{*}{No Heuristics} & Y & Y
      & 38.16 & 55.77 & 42.23 & 42.57 & 48.00 & 44.07 \\
    \cline{2-10} \\[-.8em]
    & \multirow{1}{*}{-- temporal -- coref. - keywords} & Y & N
      & 39.35 & 57.03 & 43.49 & 38.45 & 42.96 & 39.39 \\
    & \multirow{1}{*}{-- temporal -- coref.} & Y & N
      & 37.06 & 59.95 & 42.56 & 38.41 & 44.54 & 39.83 \\
    & \multirow{1}{*}{-- temporal} & Y & N
      & 39.39 & 59.53 & 44.23 & 46.81 & 52.15 & 48.23 \\
    & \multirow{1}{*}{All} & Y & N
      & 40.70 & 58.97 & 45.17 & 47.92 & 56.51 & 50.06 \\
    & \multirow{1}{*}{All} & Y & Y
      & 43.81 & 62.71 & 48.34 & 53.41 & 60.51 & 55.17 \\
    
    \midrule
    % {\color{blue}
    \multicolumn{1}{a}{\multirow{1}{*}{Human}}
    & \multicolumn{1}{a}{---} & \multicolumn{1}{a}{---} & \multicolumn{1}{a|}{---}
      & \multicolumn{1}{a}{84.74} & \multicolumn{1}{a}{81.32} & \multicolumn{1}{a|}{82.78}
      & \multicolumn{1}{a}{71.90} & \multicolumn{1}{a}{82.51} & \multicolumn{1}{a}{75.53} \\

    \bottomrule
    
    \end{tabular}
}
\caption{
\footnotesize
\textbf{Annotated-test-set performance on Instructables.com:} Similar trend is observed as in~\tbref{tab:main_dev_results_wikihow}. Note that both the \textit{Finetuned} and the \textit{Self}-training are done on the WikiHow training set and a zero-shot transfer to Instructables is performed.
}
\label{tab:main_results_instructables}
\end{table*}
